Active Learning of Probabilistic Movement Primitives

A Probabilistic Movement Primitive (ProMP) defines a distribution over trajectories with an associated feedback policy. ProMPs are typically initialized from human demonstrations and achieve task generalization through probabilistic operations. However, there is currently no principled guidance in the literature to determine how many demonstrations a teacher should provide and what constitutes a "good" demonstration for promoting generalization. In this paper, we present an active learning approach to learning a library of ProMPs capable of task generalization over a given space. We utilize uncertainty sampling techniques to generate a task instance for which a teacher should provide a demonstration. The provided demonstration is incorporated into an existing ProMP if possible, or a new ProMP is created from the demonstration if it is determined that it is too dissimilar from existing demonstrations. We provide a qualitative comparison between common active learning metrics; motivated by this comparison we present a novel uncertainty sampling approach named Greatest Mahalanobis Distance. We perform grasping experiments on a real KUKA robot and show our novel active learning measure achieves better task generalization with fewer demonstrations than a random sampling over the space.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\td{Discuss that we are looking at a specific state and context variable
combination that gives us a reasonably straight forward transformation between
the context variables and the ProMP state. We are avoiding making our approach
over-generalized, but it may be worth mentioning that if you can provide an
analytic transformation function between state and context variables then our
method can accommodate it.}


==> experiment_num_demos_fig.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{../imgs/trial_results.pdf}
  \caption{\td{This is bogus data. Need to tweak colors a bit, I think the
  darkest one is too dark and it's hard to see the middle line when printed.}}
  \label{fig:results}
\end{figure}

==> graphical_model_fig.tex <==
\begin{figure}[t]
  \centering
  \tikz{ %
  \node[latent] (w) {$\bm{w}_n$} ; %
  \node[latent, left=of w, xshift=-2cm] (pi) {$\pi$} ; %
  \node[latent, left=of w, yshift=0.7cm] (mu) {$\bm{\mu}_{\bm{w}}^m$} ; %
  \node[latent, left=of w, yshift=-0.7cm] (sigma_w) {$\bm{\Sigma}_{\bm{w}}^m$} ; % 
  % \node[latent, below=of sigma_w, xshift=-0.7cm] (alpha) {$\alpha_m$} ; %
  % \node[latent, below=of sigma_w, xshift=0.7cm] (lambda) {$\lambda_m$} ; %
  \node[obs, right=of w] (y) {$\bm{y}_t$} ; %
  \node[latent, above=of y] (sigma_y) {$\bm{\Sigma}_{\bm{y}}$} ; %
  % \node[latent, right=of sigma_y] (beta) {$\beta$} ; %
  \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate1} {(y)} {$T$}; %
  \plate[inner sep=0.25cm, xshift=-0.12cm, yshift=0.12cm] {plate2} {(w) (plate1)} {$N$}; %
  \plate {plate3} {(mu) (plate2)} {$M$}; %
  \edge {pi} {mu} ; %
  \edge {pi} {sigma_w} ; %
  \edge {mu} {w} ; %
  \edge {sigma_w} {w} ; %
  % \edge {alpha} {sigma_w} ; %
  % \edge {lambda} {sigma_w} ; %
  \edge {w} {y} ; %
  \edge {sigma_y} {y} ; %
  % \edge {beta} {sigma_y} ; %
  }
  \caption{Graphical model for our method of learning a mixture of
  ProMPs. \td{Is this still up to date?}}
  \label{fig:graphical_model}
\end{figure}
